Modelling of AC/DC Interactions of Converter-Interfaced Resources for Harmonic Power-Flow Studies in Microgrids

Power distribution systems experience a large-scale integration of Converter-Interfaced Distributed Energy Resources (CIDERs). As acknowledged by recent literature, the interaction of individual CIDER components and different CIDERs through the grid can lead to undesirable amplification of harmonic frequencies and, ultimately, compromise the distribution system stability. In this context, the interaction of the DC and AC sides of CIDERs has been shown to have a significant impact. In order to analyze and support the mitigation of such phenomena, the authors of this paper recently proposed a Harmonic Power-Flow (HPF) framework for polyphase grids with a high share of CIDERs. The framework considers the coupling between harmonics, but ignores the DC-side response of the CIDERs. Modelling the DC side and AC/DC converter introduces a nonlinearity into the CIDER model that needs to be approximated for the numerical solution of the HPF. This paper extends the CIDER model and HPF framework to address this aspect, whose inclusion is non-trivial. The extended HPF method is applied to a modified version of the CIGRE low-voltage benchmark microgrid. The results are compared to (i) time-domain simulations with Simulink, (ii) the predecessor of the extended HPF which neglects the DC side, and (iii) a classical decoupled HPF.

==> Tables/Nomenclature_PQ_CIDER.tex <==

\begin{tabularx}{\columnwidth}{p{3cm}p{5cm}}
    \hline
    \multicolumn{2}{c}{Grid-Following \CIDER}\\
    \hline
\end{tabularx}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$(\cdot)_{+/-/0}$}]
    \item[$\epsilon$] 
        The \DC equivalent of the \CIDER
    \item[$\delta$] 
        The \DC filter stage of the \CIDER
    \item[$\act$]
        The actuator of the \CIDER
    \item[$\theta$]
        A given reference angle
    \item[$\trafo_{\ctrl|\pwr}$]
        A change of reference frame from $\pwr$ to $\ctrl$
    \item[$\mathbf{T}_{\ctrl|\pwr}(t)$] 
        The \LTP matrix which describes $\trafo_{\ctrl|\pwr}$
    \item[$\mathbf{T}_{\ctrl|\pwr,h}$]
        The Fourier coefficient of $\TP_{\pwr|\grd}$ ($h\in\harmonics$)
    \item[$\hat{\mathbf{T}}_{\ctrl|\pwr}$]
        The Toeplitz matrix composed of the $\hat{\mathbf{T}}_{\ctrl|\pwr,h}$
    \item[$\mathbf{x}(t)$]
        The state vector of a state-space model
    \item[$\mathbf{u}(t)$]
        The input vector of a state-space model
    \item[$\mathbf{y}(t)$]
        The output vector of a state-space model
    \item[$\mathbf{w}(t)$]
        The disturbance vector of a state-space model
    \item[$\mathbf{A}(t)$]
        The system matrix of an \LTP system
    \item[$\mathbf{B}(t)$]
        The input matrix of an \LTP system
    \item[$\mathbf{C}(t)$]
        The output matrix of an \LTP system
    \item[$\mathbf{D}(t)$]
        The feed-through matrix of an \LTP system
    \item[$\mathbf{E}(t)$]
        The input disturbance matrix of an \LTP system
    \item[$\mathbf{F}(t)$]
        The output disturbance matrix of an \LTP system
    \item[$V_\spt$]
        The voltage setpoint of a grid-forming resource
    \item[$S_\spt$]
        The power setpoint of a grid-following resource
    \item[$v_{\grd,\cmpD}(t)$]
        The direct component of $v_{\grd}$
    \item[$v_{\grd,\cmpQ}(t)$]
        The quadrature component of $v_{\grd}$
    \item[$\xi_\cmpD(t)$]
        The time-variant signal content of $v_{\grd,\cmpD}(t)$
    \item[$V_{\grd,\cmpD,h}$]
        The Fourier coefficient of $v_{\grd,\cmpD}(t)$ ($h\in\harmonics$)
\end{IEEEdescription}
\hrule
